Electrolytes structure near electrodes with molecular size roughness

Understanding the electrodes' surface morphology influence on the ions' distribution is essential for designing the supercapacitors with enhanced energy density characteristics. We develop a model for the structure of electrolytes near the rough surface of electrodes. The model describes an effective electrostatic field's increase and associated intensification of ions' spatial separation at the electrode-electrolyte interface. These adsorption-induced local electric and structure properties result in notably increased values and sharpened form of the DC dependence on the applied potential. Such capacitance behavior is observed in many published simulations, and its description is beyond the capabilities of the established flat-electrodes theories. The proposed approach could extend the quantitatively verified models providing a new instrument of the electrodes surface-parameters optimization for specific electrolytes.

==> sections/conclusions.tex <==
%\section{conclusions}
In conclusion, we developed theory describing the ions distribution structure and accounting for the realistic roughness of the electrodes. 
Our model predicts the significant capacitance increase induced by ions-scale roughness. 
We observed that the shape of the differential capacitance dependency on applied potential changes notably with variation of roughness and becomes sharper as the roughness increases. 
Such behaviour is in agreement with the published MD simulations for the ionic liquids near well-defined heterogeneous surfaces \cite{vatamanu2011influence,xing2012nanopatterning}. 
%In contrast with the MD studies \cite{vatamanu2011influence,xing2012nanopatterning,hu2013molecular,vatamanu2014influence, bedrov2015ionic, vatamanu2017charge} using the deterministic geometries, we model the random pore wall surface. This approach makes our model suitable for the description of natural and artificially modified materials. 
The proposed method is semi-analytical and involves the numerical calculations to solve Poisson equation only, that allows to investigate the explicit geometry influence on the ionic structure. The simplicity of the approach and a wide acceptance of the used roughness model are strong advantages of our theory in comparison with the published simulations. Combining our approach with the quantitatively approved methods (such as c-DFT) is perspective to design the electrodes morphology corresponding to the desired energy/power characteristics.
%novelty
%comparison with MD
%simplicity


